Tracing Forum Posts to MOOC Content using Topic Analysis

Massive Open Online Courses are educational programs that are open and accessible to a large number of people through the internet. To facilitate learning, MOOC discussion forums exist where students and instructors communicate questions, answers, and thoughts related to the course. The primary objective of this paper is to investigate tracing discussion forum posts back to course lecture videos and readings using topic analysis. We utilize both unsupervised and supervised variants of Latent Dirichlet Allocation (LDA) to extract topics from course material and classify forum posts. We validate our approach on posts bootstrapped from five Coursera courses and determine that topic models can be used to map student discussion posts back to the underlying course lecture or reading. Labeled LDA outperforms unsupervised Hierarchical Dirichlet Process LDA and base LDA for our traceability task. This research is useful as it provides an automated approach for clustering student discussions by course material, enabling instructors to quickly evaluate student misunderstanding of content and clarify materials accordingly.

==> Makefile <==
NAME=main
#NAME=paper-diffsubmited-to-emse-1
BIBTEX=bibtex
LATEX=latex
VIEWER=`cat ~/.viewer || which okular || which evince || which open`
LATEX_OPTS=-interaction=nonstopmode -halt-on-error

VPATH=.:figures:figs:autofigs
FIGS=$(wildcard ./figures/*.png) $(wildcard ./figures/*.pdf)
CROPS=


JPGS=$(patsubst %.jpg,%.eps,$(filter %.jpg,$(FIGS)))
GIFS=$(patsubst %.gif,%.eps,$(filter %.gif,$(FIGS)))
PNGS=$(patsubst %.png,%.eps,$(filter %.png,$(FIGS)))
SVGS=$(patsubst %.svg,%.eps,$(filter %.svg,$(FIGS)))
PDFS=$(patsubst %.pdf,%.eps,$(filter %.pdf,$(FIGS)))

EPSS=$(addsuffix .eps,$(basename $(FIGS)))


.PHONY: all clean default view push commit zip

default: view

all: $(NAME).pdf

$(NAME).pdf: *.cls $(NAME).tex *.bib $(EPSS) $(CROPS)
	echo $(EPSS)
	$(LATEX) $(LATEX_OPTS) $(NAME).tex
	@if(grep "There were undefined references" $(NAME).log > /dev/null);\
	then \
		$(BIBTEX) $(NAME); \
		$(LATEX) $(LATEX_OPTS) $(NAME).tex; \
	fi
	@if(grep "Rerun" $(NAME).log > /dev/null);\
	then \
		$(LATEX) $(LATEX_OPTS) $(NAME).tex;\
	fi
	$(LATEX) $(LATEX_OPTS) $(NAME).tex
	dvips -j0 -Ppdf -Pbuiltin35 -G0 -z $(NAME).dvi
	gs -q -dPDFA \
	-dNOPAUSE -dBATCH -dSAFER -dPDFSETTINGS=/prepress \
	-dAutoFilterColorImages=false \
	-dAutoFilterGrayImages=false \
	-dAutoFilterMonoImages=false \
	-dColorImageFilter=/FlateEncode \
	-dGrayImageFilter=/FlateEncode \
	-dMonoImageFilter=/FlateEncode \
	-sDEVICE=pdfwrite -sOutputFile=$(NAME).pdf \
	-c .setpdfwrite \
	-f $(NAME).ps





clean:
	rm *.blg *.bbl *.log *.aux $(NAME).pdf $(NAME).dvi $(NAME).ps || echo Already Clean

view:	$(NAME).pdf
	$(VIEWER) $(NAME).pdf

$(SVGS) : %.eps : %.svg
	inkscape -b white -t -T --export-ignore-filters --export-eps=$@ $<

# Use PS pipeline for maximum compatibility with random latex packages

$(JPGS) : %.eps : %.jpg
	anytopnm $< | pnmtops -nocenter -equalpixels -dpi 72 -noturn -rle -setpage - > $@
$(GIFS) : %.eps : %.gif
	anytopnm $< | pnmtops -nocenter -equalpixels -dpi 72 -noturn -rle -setpage - > $@
$(PNGS) : %.eps : %.png
	anytopnm $< | pnmtops -nocenter -equalpixels -dpi 72 -noturn -rle -setpage - > $@



%-crop.pdf: %.pdf
	pdfcrop $<

%-crop.eps: %-crop.pdf
	pdftops -eps $< $@

$(PDFS) : %.eps : %.pdf
	pdftops -eps $< $@

push:	commit
	git push

commit:	
	git commit -av

zip : $(NAME).zip

$(NAME).zip : *.cls $(NAME).tex *.bib $(EPSS) Makefile
	zip $@ $^

x: $(NAME).pdf
	xournal $(NAME).pdf



==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)
